Processing stationary noise: model and parameter selection in variational methods

Additive or multiplicative stationary noise recently became an important issue in applied fields such as microscopy or satellite imaging. Relatively few works address the design of dedicated denoising methods compared to the usual white noise setting. We recently proposed a variational algorithm to tackle this issue. In this paper, we analyze this problem from a statistical point of view and provide deterministic properties of the solutions of the associated variational problems. In the first part of this work, we demonstrate that in many practical problems, the noise can be assimilated to a colored Gaussian noise. We provide a quantitative measure of the distance between a stationary process and the corresponding Gaussian process. In the second part, we focus on the Gaussian setting and analyze denoising methods which consist of minimizing the sum of a total variation term and an $l^2$ data fidelity term. While the constrained formulation of this problem allows to easily tune the parameters, the Lagrangian formulation can be solved more efficiently since the problem is strongly convex. Our second contribution consists in providing analytical values of the regularization parameter in order to approximately satisfy Morozov's discrepancy principle.

==> Notes_Supplementaires.tex <==
\subsection{Polynomial behaviors}


We further assume that:
$$
\psi(x)\leq \frac{M}{|x|^\beta}.
$$
and 
$$
\psi(x)\geq \frac{m}{|x|^\beta}.
$$
where $\beta,M,m>0$ and $|x|>\epsilon>0$. 

We may wonder which $\beta$ ensures convergence to a Normal distribution as $n\rightarrow+\infty$. 
Since we assume that $\Lambda$ is an i.i.d. random vector with $0$ mean, convergence will occur for any choice of the marginals of $\Lambda$. 
We thus only look for a condition on $\beta$.

Let us denote:
$$
f(R)=\frac{\int_{B(0,R) \backslash B(0,\epsilon)}|\psi|^3(x) dx}{\left(\int_{B(0,R)\backslash B(0,\epsilon)}|\psi|^2(x) dx\right)^{3/2}}.
$$
Note that $\frac{\sum_{i=1}^n \rho_i}{(\sum_{i=1}^n \sigma_i^2)^{3/2}}$ in equation \eqref{eq:Berry} is just a Riemann approximation of $f(R)$ for a certain $R$.

The integrals can be computed explicitely using polar coordinates: 
\begin{align*}
\int_{B(0,R)\backslash B(0,\epsilon)}|\psi|^2(x) dx &\geq 2\pi m^2\int_{\epsilon}^R  \frac{1}{r^{2\beta}} r dr \\ 
&= 2\pi m^2 \left[\frac{r^{2-2\beta}}{2-2\beta}\right]_{\epsilon}^{R}
\end{align*}
This quantity will tend to $+\infty$ if $2-2\beta>0$, i.e. $\beta<1$. In that case:
$$
\left(\int_{B(0,R)\backslash B(0,\epsilon)}|\psi|^2(x) dx \right)^{3/2}\stackrel{R=+\infty}{\sim} R^{3-3\beta}c.
$$
with $c>0$. Similarly:
\begin{align*}
\int_{B(0,R)\backslash B(0,\epsilon)}|\psi|^3(x) dx &\leq 2\pi M^3\int_{\epsilon}^R  \frac{1}{r^{3\beta}} r dr \\ 
&= 2\pi M^3 \left[\frac{r^{2-3\beta}}{2-3\beta}\right]_{\epsilon}^{R}.
\end{align*}

Looking at these expressions, we get that the upper bound in \eqref{eq:Berry} goes to $0$ as long as $\beta<1$.
Finally, we get the result:

\begin{center}
 For any kernel $\psi$ decaying to $0$ slowlier than $\frac{1}{|x|}$, the noise distribution is Gaussian whatever the marginals of $\Lambda$ (for an infinite number of pixels).
\end{center}

Je ne sais pas trop ce qui se passe lorsque le filtre peut prendre des valeurs positives et n\'egatives. Par exemple pour l'image du Baboon j'ai utilis\'e un sinus cardinal.

\subsection{The case of a Bernoulli-Uniform noise + a Gaussian kernel}

This is the kind of distribution which would lead to ``sparse'' signals. 
\footnote{I guess that Bernoulli-Gaussian or Bernoulli-Laplace distributions would lead to the same kinds of bound.} 

It satisfies:
$$
p(\Lambda(y)\neq 0)=\alpha.
$$
$$
p(\Lambda(y)=0)=1-\alpha.
$$
and 
$$
\Lambda(y)|\Lambda(y)\neq 0 \sim U([-1,1]).
$$

For this distribution, we have:
$$
\E(\Lambda(y))=0,
$$
$$
\sigma^2=\E(\Lambda^2(y))=\alpha \int_{-1}^1x^2dx = \frac{2}{3}\alpha,
$$
and
$$
\rho=\E(|\Lambda(y)|^3)=2\alpha \int_{0}^1x^3dx = \frac{\alpha}{2}.
$$

Now, let us set:
$$
\psi(x_1,x_2)=\frac{1}{2\pi \sigma_1\sigma_2}\exp\left( - \frac{x_1^2}{\sigma_1^2}- \frac{x_2^2}{\sigma_2^2}\right).
$$
This corresponds to what is used in our experiments.

We want to assess the distance from $B(0)$ to the Normal distribution. We have:
$$
\E(\Lambda(y)\psi(x-y))=0,
$$
$$
\sigma^2(x-y)=\E(\Lambda^2(y)\psi(x-y))=\frac{2}{3}\alpha \psi^2(x-y),
$$
and
$$
\rho(x-y)=\E(|\Lambda(y)\psi(x-y)|^3)=\frac{\alpha}{2}|\psi|^3(x-y).
$$

These quantities can be replaced in \eqref{eq:Berry} leading to:
$$
\|F_n-\Phi\|_\infty\leq \frac{C_1}{\sqrt{\alpha}} \frac{\sum_{x} |\psi(x)^3|}{(\sum_{x} \psi(x)^2)^{3/2}}.
$$
where $F_n$ is the distribution function of $B(0)$ and $C_1=\frac{1}{2}C_0\left( \frac{2}{3}\right)^{-3/2}$.

We use the approximations:
$$
\sum_{x} |\psi|^3(x-y)\simeq \int_{\mathbb{R}^2}|\psi|^3(x-y)dy_1dy_2 
$$
and 
$$
\sum_{y_1,y_2} \psi^2(y_1,y_2)\simeq \int_{\mathbb{R}^2}\psi^2(y_1,y_2)dy_1dy_2. 
$$
These integrals can be computed exactly:
$$
\int_{\mathbb{R}^2}|\psi|^3(x-y)dy_1dy_2=\frac{1}{12\pi \sigma_1^2\sigma_2^2}
$$
and
$$
\int_{\mathbb{R}^2}|\psi|^2(x-y)dy_1dy_2=\frac{1}{4\pi \sigma_1\sigma_2}.
$$

Overall we get that (sauf erreur):
\begin{equation}
\|F_n-\Phi\|_\infty\leq \frac{C_2}{\sqrt{\alpha}} \sqrt{\frac{\pi}{\sigma_1\sigma_2}}. 
\end{equation}

where $C_2=\frac{2}{3}C_1$. Looking at this expression we see that:
\begin{itemize}
 \item In the case $\alpha=1$, $\Lambda$ has a uniform distribution. This analysis thus covers the cases of white uniform processes and the class of Bernoulli-Uniform signals.
 \item The sparsest the signal (i.e. the smaller $\alpha$), the least accurate the Gaussian approximation. 
However, this does not look too bad since there is a $\sqrt{\cdot}$ on $\alpha$. 
 \item Both $\sigma_1$ and $\sigma_2$ should be ``far'' from $0$ to get a good approximation. This is not too good... 
 \item It could be interesting to evaluate these values numerically for typical values of $\sigma_1$ and $\sigma_2$.
\end{itemize}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{1D}

Let $(\psi(k))_{k\in \N^*}$ denote a sequence of kind $\psi(k)=k^m, \ m\in \N$.
The truncated serie $\sum_{k=1}^N \psi(k)^m$ satisfies:
$$\sum_{k=1}^N \psi(k)^m\sim C(m) N^{m+1}$$
where $C(m)>0$ only depends on $m$.

Thus by denoting 
$$
f(N)=\frac{\sum_{k=1}^N \psi(k)^3}{(\sum_{k=1}^N \psi(k)^2)^{3/2}},
$$
we get:
$$
\lim_{N\rightarrow +\infty} f(n) = \lim_{N\rightarrow +\infty} \frac{C(3m+1) N^{3m+1}}{ C(2m+1) N^{3m+3/2}}=0.
$$
We can thus state the following result:
\begin{proposition} 
Let $\lambda_n$ denote an i.i.d. random vector of size $n$. We assume that the marginals of $\lambda_n$ have finite variance and third order moments. 
Let $\psi_n=(\psi(k))_{k=1}^n$.
For all sequences of kind $\psi(k) = k^m$, $m \in \N$, the random variable:
$$
b_n=\lambda_n\times \psi_n
$$
converges in law to a gaussian vector $\mathcal{N}(0,\mathcal{F}^{-1}\mathop{diag}(|\hat \psi|^2) \mathcal{F})$ as $n$ goes to infinity.
\end{proposition}

By a similar reasoning obtained by comparing the serie to an integral, we get:
\begin{proposition} 
For all kernels satisfying $|\psi(k)|\sim k^\alpha$, $\alpha \geq -1/2$, the random variable:
$$
b_n=\lambda_n\times \psi_n
$$
converges in law to a gaussian $\mathcal{N}(0,\mathcal{F}^{-1}\mathop{diag}(|\hat \psi|^2) \mathcal{F})$.
\end{proposition}

Looking at the above result, it seems possible that $f(n)$ goes to $0$ as long as $\sum_{k=1}^N \psi(k)^2$ diverges. 
This would be nice!

\subsection{What happens in higher dimensions}

